Addressing Limited Data for Textual Entailment Across Domains

We seek to address the lack of labeled data (and high cost of annotation) for textual entailment in some domains. To that end, we first create (for experimental purposes) an entailment dataset for the clinical domain, and a highly competitive supervised entailment system, ENT, that is effective (out of the box) on two domains. We then explore self-training and active learning strategies to address the lack of labeled data. With self-training, we successfully exploit unlabeled data to improve over ENT by 15% F-score on the newswire domain, and 13% F-score on clinical data. On the other hand, our active learning experiments demonstrate that we can match (and even beat) ENT using only 6.6% of the training data in the clinical domain, and only 5.8% of the training data in the newswire domain.

==> challenges.tex <==
\section{Challenges with clinical data}
\label{sec:challenges}

Clinical narratives are written by healthcare professionals in a practice setting. These are substantially different from newswire text, which is consistent and well-formed in terms of English grammar, spellings and punctuation. Clinical notes are characterized by misspellings, abbreviations, incomplete sentences, inconsistent document structure, embedded semi-structured content (see Figure \ref{fig:sampleNote}), and other undesirable properties of poor text quality. This poses a significant challenge to NLP systems \cite{Meystre2008}. Owing to the lack of punctuation, identifying sentence boundaries is not straightforward in clinical text. We used the approach described in \cite{mccord2012} to identify sentence boundaries and calculated sentence length of each sentence in terms of number of words. The distribution for sentence length is significantly different for the development set of our clinical text ($\mu=7.74$ and $\sigma=7.85$) as compared to that of the development set for RTE-5 pilot data ($\mu=21.4$ and $\sigma=10.59$). This illustrates that clinical text and newswire text in RTE data are substantially different.

Another characteristic our annotators found in our data was that two or more sentences together were allowed to conclude entailment, but either one by itself was not sufficient to do so. For example: Consider the hypothesis: ``The patient has a history of diabetes.'' The progress note (see Figure \ref{fig:sampleNote}) that allowed annotators to conclude that this hypothesis was true, had a section titled ``Past Medical History''.
\begin{figure}
	\noindent\fbox
	{
		\begin{minipage}{0.94\linewidth}
			\texttt{**NAME[XX (YY) ZZ]  has no liver problems.}\\
			\texttt{PAST MEDICAL HISTORY}\\					
			\texttt{1. Htn}\\			
			\texttt{Well controlled}\\
			\texttt{2. Diabetes mellitus}\\			
			\texttt{On regular dose of insulin.}\\
			\\
			\texttt{FAMILY HISTORY:}\\
			\texttt{Father with T2DM age unknown}
		\end{minipage}
	}
\caption{Excerpt from a sample clinical note.}
\label{fig:sampleNote}
\end{figure}
 Listed within the section are multiple disorders, including diabetes, with one-sentence descriptions for each.  In order to conclude that the hypothesis is true, the annotators required evidence from both the section heading and the sentence that stated diabetes. Our parser identified each line in Figure \ref{fig:sampleNote} as a separate sentence. In this case our annotators annotated entailment relationship for  the section heading ``Past Medical History'', and the sentence that mentioned diabetes ``2. Diabetes mellitus'', and marked no entailment relationship for other sentences. 

This characteristic is very similar to the phenomenon of \textit{partial entailment} discussed by  \newcite{levy2013} , where a hypothesis can be broken down into one or more elements and text entails some of the elements, but not the hypothesis. It should be noted that the phenomenon of partial entailments is not found in RTE data, and makes the task of textual entailment search even harder. We discuss partial entailments in our dataset in Section \ref{sec:discussion}.






==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

